Quasi-Optimal Partial Order Reduction

A dynamic partial order reduction (DPOR) algorithm is optimal when it always explores at most one representative per Mazurkiewicz trace. Existing literature suggests that the reduction obtained by the non-optimal, state-of-the-art Source-DPOR (SDPOR) algorithm is comparable to optimal DPOR. We show the first program with $\mathop{\mathcal{O}}(n)$ Mazurkiewicz traces where SDPOR explores $\mathop{\mathcal{O}}(2^n)$ redundant schedules and identify the cause of the blow-up as an NP-hard problem. Our main contribution is a new approach, called Quasi-Optimal POR, that can arbitrarily approximate an optimal exploration using a provided constant k. We present an implementation of our method in a new tool called Dpu using specialised data structures. Experiments with Dpu, including Debian packages, show that optimality is achieved with low values of k, outperforming state-of-the-art tools.

==> src/02-overview.tex <==
%!TEX root = ../main.tex

\section{Overview and Motivating Example}
\label{sec:overview}

\todo{Rename to "Illustrative examples"}
\cro{We think we should instead combine sections 1 and 2 into 1 single section,
   they are currently consuming 5 pages!}

% \includegraphics[scale=0.75]{fig/ssbexp.fig}
\begin{figure*}[t]
\centering
\begin{tabular}[b]{lll}
%\toprule
	\scalebox{0.7}{
	\rotatebox{90}{
	\parbox[b]{6cm}{
		(a)
		\begin{tabular}{ccccc}
			$w_0$ & $w_1$ & $w_2$ & count & master \\
			\hline
			$x_0=7$ & $x_1=8$ & $x_2=9$ & $c=1$ & $i=c$ \\
			& & & $c=2$ & $x_i=0$
		\end{tabular}
	} %parbox
	} %rotatebox
	} %scalebox	
&
	\scalebox{0.6}{(b) \input{fig/ssbexpf.tex}}
&	
	\quad
	\scalebox{0.6}{
	\begin{tabular}[b]{l}
		\parbox[b]{4cm}{
		\begin{tabular}{ccc}
			$w$ & $r$ & $r'$ \\
			\hline
			$x=1$ & $y=x$ & $z=x$
		\end{tabular}
		(c)
		}
		\smallskip
		\\
		\parbox[b]{4cm}{
		\begin{tabular}[b]{c}
			$\indep \eqdef \set{(r,r'),(r',r)}$\\
			$\inter{\set{1,2,3}}=\set{wrr',wr'r}$
		\end{tabular}
		(d)
		} %parbox
		\smallskip
%		\\
%		\parbox[b]{3cm}{
%		(d) \input{fig/ssbexpd.tex}
%		}
		\smallskip
		\\
		\parbox[b]{4cm}{
		\input{fig/ssbexpe.tex}
		(e)
		}
	\end{tabular}
} % scalebox	
%\\
%\bottomrule
\end{tabular}
\caption{Programs, partially ordered executions and unfolding.\\
	Boxes are events named by its order of appearance in the unfolding}
\label{fig:exunf}
\end{figure*}


%\scalebox{0.8}{
%\parbox[b]{6cm}{
%(a)
%\begin{tabular}{ccccc}
%$w_0$ & $w_1$ & $w_2$ & count & master \\
%\hline
%$x_0=7$ & $x_1=8$ & $x_2=9$ & $c=1$ & $i=c$ \\
% & & & $c=2$ & $x_i=0$
%\end{tabular}
%} %parbox
%
%%\smallskip
%%\parbox[b]{3cm}
%%{
%%(c)
%%\begin{tabular}{c}
%%$\indep \eqdef \set{(r,r'),(r',r)}$\\
%%$\inter{\set{1,2,3}}=\set{wrr',wr'r}$
%%\end{tabular}
%%} %parbox
%
%} %scalebox

%\qquad
%\scalebox{0.6}{(d) \input{fig/ssbexpd.tex}}
%\qquad
%\scalebox{0.6}{(e) \input{fig/ssbexpe.tex}}
%
%\medskip

%\scalebox{0.5}{(f) \input{fig/ssbexpf.tex}}
%
%\smallskip
%\parbox[t]{6cm}
%{
%	(b)
%	\begin{tabular}{ccc}
%		$w$ & $r$ & $r'$ \\
%		\hline
%		$x=1$ & $y=x$ & $z=x$
%	\end{tabular}
%}
%\scalebox{0.6}{(e) \input{fig/ssbexpe.tex}}
%}

\todo{- change the figure labels and corresponding texts.\\
- Explain the numbers in the boxes in caption}

%\begin{figure}[t]
%\centering
%\begin{center}
%\input{fig/overview-ssb}
%\end{center}
%\caption{Execution tree explored by SDPOR on the program shown
%in~\cref{fig:exunf}~(a).}
%\label{fig:sdpor}
%\end{figure}

Consider the program shown in~\cref{fig:exunf}~(a).
%
It contains three~\emph{writer} threads $w_0, w_1, w_2$, each writing
to a different variable.
%
The thread~\emph{count} increments a counter~$c$, initialized with~0.
%
Thread~\emph{master} reads the counter into variable~$i$, then writes to 
variable~$x_i$.
%
%This program can naturally be generalized to~$n$~\emph{writer} threads instead 
%of~3, where the \emph{counter} thread would count to~$n$ and no change would be 
%necessary in the \emph{master} thread.
The natural extension to~$n$~\emph{writers} would only modify the count thread.

PORs exploit the \emph{independence} of statements.
%
For example, statements $x_0 = 7$ and $x_1 = 8$ are independent because they 
produce the same state regardless of their order of execution.
%
Statements $i = c$ and any statement in the~\emph{count} thread are dependent 
or~\textbf{race} (conflict) \hn{conflict???}, as their execution order results in a different state.
%
Similarly $x_i = 0$ races with exactly one of the~\emph{writer} threads, 
depending on the value of~$i$.

The set of executions of this program can be partitioned into 6~different 
classes, corresponding to the 6~partial orders shown in~\cref{fig:exunf}~(b).
% \lp{In the figure we mix the name of the thread ($w_i$) and statements that are executed
% (\eg $i=0$). Also $x_i=2$ should be $x_i=0$. I can make the corrections if ok with
% you.}
%
This classification is defined by the equivalence relation $\equiv$ on the set 
of executions, where two executions are equivalent if we can construct the 
second execution from the first by swapping adjacent independent statements.
%
Equivalent executions are topological sortings of the same partial order
(\emph{dependency graphs})
%
%These partial orders, called \emph{dependency graphs}, 
These are constructed based on 
a happens-before relation between dependent statements.
%
A POR is optimal when it explores exactly one execution per equivalence class.
%
In this program, an optimal POR explores 6~executions ($2n$-executions for~$n$ \emph{writers})
%and in the 
%generalisation of the program to~$n$ \emph{writer} threads, it would 
%explore~$2n$-executions as~$\equiv$ would have exactly~$2n$ equivalence 
%classes.
%We now explain why the SDPOR algorithm would instead explore~$\bigo{2^n}$. 
%
SDPOR algorithm would instead explore~$\bigo{2^n}$. In short, SDPOR is a loop that
(1) executes the program until termination,
(2) finds two racing statements that can be swapped, and
(3) reverses them and re-executes the program.
%
SDPOR terminates when no more races can be swapped.

Consider the data races on the counter variable~$c$ between the~\emph{master} 
and the~\emph{count} thread.
%
%Crucially, in this program the order in which these are executed determines 
%which of the~\emph{writer} threads races with the~\emph{master} statement~$x_i 
%= 0$.
Their execution order determines which~\emph{writer} thread races with the~\emph{master} statement~$x_i= 0$.
%
If $c=1$ is executed just before $i=c$, then $x_i=0$ interferes with~$w_1$.
%
However, if $i=c$ is executed before, then $x_i=0$ interferes with~$w_0$.
%
Since SDPOR does not track relations between races, it will na\"ively try to 
reverse the race between $x_i=0$ and \emph{all writer threads}, which 
results in exploring~$\bigo{2^n}$ executions.
%
Exploring only 6 traces requires understanding the entanglement between both
races as the order in which one is solved determines the second race.

QPOR addresses this limitation of SDPOR by lifting the reasoning from 
sequential executions to a partial-order representation known as prime event 
structures (PES)~\cite{NPW81}. 
%

\todo{Remove from "We recall ...different states of the program" and example 1, then discuss PES in basic definitions.}
We recall event structure semantics for programs~\cite{RSSK15} using the simple 
program shown in~\cref{fig:exunf}~(b).
%
A PES is a triple $\tup{E, {<}, {\cfl}}$, where~$E$ is a set of events, $<$~is
the \emph{causality relation} between events (also known as 
the~\emph{happens-before} relation)
and~$\cfl$ is the conflict relation, which intuitively represents races.
%
The PES of a program is a compact representation of the dependency graphs of 
the program.
%
We call each element of a dependency graph labelled by a 
program statement an~\emph{event}.
%
The PES is a compact representation as we merge events from different graphs 
that are~\emph{history-equivalent}, \ie, we merge events that are labelled by 
the same statement and have the same causal predecessor events.
%
\Cref{fig:exunf}~(d) shows the dependency graphs of~\cref{fig:exunf}~(b),
and \cref{fig:exunf}~(e) the PES.
%
Equivalent events are identified by the same number.
%
The conflict relation is depicted with dotted lines and captures the fact that
two events race and are \emph{not} in the same dependency graph.
%
For instance, events~1 and~4 are in conflict because their statements race and 
they are not in the same dependency graph.
%
Observe that the set of events~$\set{2,4,10}$ represents instances of the same 
program statement in different states of the program.

%
%Now, coming back to QPOR
In QPOR, a $k$-partial alternative is nothing else than a set
of events satisfying some constraints.
%
Similar to SDPOR, the QPOR algorithm is a loop that
%
(1) executes the program until the end and transforms the execution into a
dependency graph,
%
(2) finds the next dependency graph to explore by computing the $k$-partial 
alternative to the current dependency graph, \ie, a set of events in the event 
structure that conflicts with at least~$k$ events in the dependency graph, and
%
(3) re-executes the program following the new dependency graph found in (2).
%

\todo{This part about SDPOR should be removed because it is in the introduction already}
SDPOR corresponds to (a simplification of) QPOR with $k=1$.
\cro{When combining the sections, this will get done ;)}
%
Optimal POR corresponds to $\infty$-partial alternatives.
%
Computing $\infty$-partial alternatives is NP-complete,
but computing $k$-partial alternatives, with $k \in \N$
requires $\bigo{n^k}$ time.


For the program shown in~\cref{fig:exunf}~(a), QPOR with $k=1$ would as well 
explore $\bigo{2^n}$ redundant executions. 
%\hn{$\bigo{2^n}$ is additional exe or total number}
%
However, it would perform optimal exploration (6 executions) with $k=2$ because data races are coupled with (at 
most) one other data race.

\todo{Part from "Finding and maintaining ..the number of explored executions"should be merged in the introduction.}
Finding and maintaining $k$-partial alternatives requires decision procedures 
for checking the causality and conflict relations on event structures.
%
Vector clocks are a prominent algorithm for deciding causality relations, but 
they work only when restricted to events of the same dependency 
graph~\cite{Fid88}.
%
In~\cref{sec:algo} we present data structures and algorithms that represent an
event structure as a set of causality trees. 
%
The central idea in our technique is that the causality and conflict relations 
of the event structure of a program can be efficiently represented as a set of 
trees where every event is composed of one or two nodes in two different trees.
%
%Trees intuitively represent the branching behavior of the sychronizing
%constructs of a program (global variables and program counters).
%
Our decision procedures for checking causality/conflict relations between events
reduce the decision to a search within one of the trees in the structure.
%
In~\cref{sec:exp} we experimentally evaluate the performance of these 
algorithms.
%
Our results show that this tree-based representation is particularly well 
suited to implement a POR because most of the causality/conflict queries 
performed by the POR can be answered in very short walk over the trees.

We have also implemented QPOR into an efficient stateless verification tool 
named~\dpu capable of exhaustively testing large code bases.
%
The main results of our experimental evaluation are that
%
(1) QPOR achieves optimal exploration even under very small values of $k$ and
largely outperforms SDPOR;
%
(2) \dpu  is able to exhaustively test 5 large programs coming from various
Debian packages orders of magnitude faster than testing tools and achieves much higher coverage of the state space;
%
(3) we profile~\dpu and show that the most significant factor affecting the runtime of a stateless POR is the number of explored executions.


The proofs of all formal results presented in this paper are available
in the appendix
\ifwithappendix % FULL VERSION
of this paper.
\else
of the unabridged version~\cite{AUTH}.
\fi

%The second one can be flipped only if the first one happens in one specific order.

%We explain the features that a program needs to expose for it not to be explored
%optimally for a given value of~$k$, and argue that most programs are unlikely to
%contain those features.
%
%When an optimal POR runs faster than an unoptimal one, two things are possible:
%either the possibly exponential combinatorial explosion does not happen in
%practice or the runtime penalty is in fact absorbed by the savings in terms of
%number of explored executions.

\subsection{Related Work}
\todo{To be somewhere at the beginning of the introduction}
\cro{I find introductory paragraphs of the intro well as they are. The paragraph
below in its current version does not compare our technique to others, as
remarked by the reviewers. Instead I think we shoud have a proper comparison
to other techniques.}
%\input{src/relatedwork}
Early PORs are based on the static identification of the subset of transitions 
enabled at a state~\cite{Val91,BCMDH92,God96}.
%
Even it is then combined with sleep set and dynamically computed in 
\emph{DPOR}~\cite{FG05}, persistent set do not guarantee optimal exploration.
%
Extensions of the original DPOR, include the use of vector clocks~\cite{NMR14}, 
Monotonic POR~\cite{KWG09}, source set based DPOR~\cite{AAJS14} and optimal 
DPOR~\cite{AAJS14} which use wakeup trees to prevent any sleep-set-blocked 
exploration.
%
On the other axis, the unfolding method also deals with the state space 
explosion problem by replacing full labeled transition systems by compact 
partially ordered graphs.
%
It has been traditionally developed as partial-order semantics for Petri 
Nets~\cite{MCM95,ERV02}, and more used for analysis multithreaded 
programs~\cite{SRDK17,RSSK15,KH14}.

